Information Flow in Black Hole Evaporation

Recently, new holographic models of black hole evaporation have given fresh insights into the information paradox [arXiv:1905.08255, arXiv:1905.08762, arXiv:1908.10996]. In these models, the black hole evaporates into an auxiliary bath space after a quantum quench, wherein the holographic theory and the bath are joined. One particularly exciting development is the appearance of "ER=EPR"-like wormholes in the (doubly) holographic model of [arXiv:1908.10996]. At late times, the entanglement wedge of the bath includes the interior of the black hole. In this paper, we employ both numerical and analytic methods to study how information about the black hole interior is encoded in the Hawking radiation. In particular, we systematically excise intervals from the bath from the system and study the corresponding Page transition. Repeating this process ad infinitum, we end up with a fractal structure on which the black hole interior is encoded, implementing the uberholography protocol of [arXiv:1612.00017].

==> sections/App.tex <==
% !TEX root = ../BH_v04.tex

\section{Generalized Entropy, QES and Page Curve}
The generalized entropy associated with a bulk surface $\mathcal{X}$ is defined as the sum of area and the quantum correction from the von Neumann entropy of matter term in the bulk
\begin{equation}\label{Sgen}
 S_{\text{gen}}= \frac{A\( \mathcal{X}\)}{4\GN } + S_{\text{Bulk}}\,,
\end{equation}
which is minimized by the surface called quantum extremal surface. In this $\text{AdS}_2$-bath model, the classical entropy is determined by the value of dilaton in nearly $\text{AdS}_2$ model and the bulk entropy can be calculated by taking replica trick and considering the R\'enyi entropy. Thanks to the two-dimensional CFT, the question is transfered to the calculations of expectation value of twist operators at the endpoints of the intervals. Before the coupling, the dilaton takes the simple static solution
\begin{equation}\label{dilaton01}
 \phi=2 \bar{\phi}_{r} \frac{1-\left(\pi T_{0}\right)^{2} x^{+} x^{-}}{x^{+}-x^{-}} = 2 \bar{\phi}_{r}  \pi T_0\coth\( \pi T_0 (y^+ -y^-)\) \,,
\end{equation}
where we used the reparameterization function for static Black hole with temperature $T_0$, \ie $f_0\( u \)= \frac{1}{\pi T_0} \tanh \( \pi T_0 u\)$. After the coupling with bath, the $\text{AdS}_2$ geometry is changed and decided by the new profile of dilaton. For the point after the shock $x^- >0$, the new solution is
\begin{equation}\label{dilaton02}
 \phi=2 \bar{\phi}_{r} \frac{1-\left(\pi T_{0}\right)^{2} x^{+} x^{-}  + \frac{k}{2} I\( x^+,x^-\)}{x^{+}-x^{-}} \,, \text{with} \quad I = \int_0^{x^-}(x^+-t)(x^--t)\{u,t\} dt\,,
\end{equation}
which is solved by a given tress tensor~\cite{Maldacena:2016upp,Almheiri:2014cka}. For the bulk entropy, we can first calculate it in the upper half plane (UHP)~\cite{Cardy:1984bb,Calabrese:2007rg,Coser_2014} and then map it to the physical coordinate system. The method is based on the results for two point function of twist operators on UHP
\begin{equation}
 \langle \mathcal{T}_n \(z_1\)\mathcal{T}_{-n} \(z_2\) \rangle_{\text{UHP}} = \frac{\mathcal{F}_n\( \zeta\)}{\left|\zeta \cdot (z_1-\bar{z}_1) (z_2-\bar{z}_2)) \right|^{\Delta_n}}  = \frac{\mathcal{F}_n\( \zeta\) }{\left|(1-\zeta) (z_1-z_2) (\bar{z}_1-\bar{z}_2)) \right|^{\Delta_n}} \,,
\end{equation}
where $\Delta_n = \frac{c}{12}(n-1/n)$ is the scaling dimension of twist operator, the $\zeta$ is the standard cross-ratio
\begin{equation}
 \zeta = \frac{(z_1 -z_2)(\bar{z}_1-\bar{z}_2)}{(z_1-\bar{z}_2)(\bar{z}_1-z_2)} \equiv \frac{z_{12}z_{\bar{1}\bar{2}}}{z_{1\bar{2}}z_{\bar{1}2}} \quad \in [0,1] \,, \(1-\zeta \equiv (-)\frac{(z_1-\bar{z}_1)(z_2-\bar{z}_2)}{(z_1-\bar{z}_2)(\bar{z}_1-z_2)}\)
\end{equation}
and function $\mathcal{F}$ only depending on the invariant cross-ratio is not universal and varies for different CFT theories. The cluster decomposition limits only fix the following condition
\begin{equation}
 \mathcal{F}_n  \longrightarrow 1\,, \text{when}   \qquad \zeta \longrightarrow 0, 1\,.
\end{equation}
However, it is found that even the four point function on the full plane is not also universal but will reduce to a universal form after taking the  large $c$ limit which implies that we can expect the holographic CFT will have a simpler results for also two point function on the UHP. In the limit $c \rightarrow \infty$, the universal four-point function on the full-plane is due to the fact that~\cite{Hartman:2013mia} the  conformal block decomposition always factorizes in either the s-channel or t-channel where the sharp phase transition happens at $\zeta= \frac{1}{2}$ \footnote{Here except for the large $c$ limit, we also need to assume the CFT only has a sparse spectrum, \ie the number of operator not scale with the $c$. And we should also expect the transition for general CFT should be very smooth due to the finite $c$ contributions from the two channels.}. According to the standard image method~\cite{Cardy:1984bb,DiFrancesco:1997nk}, the two point function on UHP for holographic CFT is also fixed to be
\begin{equation}
 \langle \mathcal{T}_n \(z_1\)\mathcal{T}_{-n} \(z_2\) \rangle_{\text{UHP}} =_{c-\rightarrow \infty}
 \begin{cases}
  \frac{1}{\left| (z_1-\bar{z}_1) (z_2-\bar{z}_2)) \right|^{\Delta_n}}\,, \qquad  \zeta \in [\frac{1}{2}, 1] \\
  \,                                                                                                         \\
  \frac{1}{\left| (z_1-z_2) (\bar{z}_1-\bar{z}_2)) \right|^{\Delta_n}}\,, \qquad \zeta \in [0,\frac{1}{2}]   \\
 \end{cases}\,,
\end{equation}
where we use the factorized function $\mathcal{F}$ in large $c$ limit, \ie
\begin{equation}
 \mathcal{F}_n \( \zeta\) = \begin{cases}
  \zeta^{\Delta_n}\,, \qquad  \zeta \in [\frac{1}{2}, 1]   \\
  (1-\zeta)^{\Delta_n}\,, \qquad \zeta \in [0,\frac{1}{2}] \\
 \end{cases}\,.
\end{equation}
The above universal results lead us to the von Neumann entropy with two endpoints on UHP as
\begin{equation}\label{Sn=1}
 S_{\text{UHP}}=S_{n\rightarrow 1} = \begin{cases}
  \frac{c}{6} \log \( |z_1-z_2|\cdot|\bar{z}_1 -\bar{z}_2|\) \,, \qquad  \zeta \in [0,\frac{1}{2}]\,, \\
  \frac{c}{6} \log \( |z_1-\bar{z}_1|\cdot|z_2 -\bar{z}_2|\)\,, \qquad \zeta \in [\frac{1}{2},1]\,,   \\
 \end{cases}
\end{equation}
which is shown in figure~\ref{UHP_plot} and which will be used to calculate the bulk entropy in generalized entropy. This result (with UV cut off) also matches the holographic entanglement entropy from Ryu-Takayanagi formula~\cite{Rangamani:2016dms} and also the holographic BCFT model with tensionless brane~\cite{Takayanagi:2011zk,Fujita:2011fp}.

\begin{figure}[t]
 \centering\includegraphics[width=3.50in]{UHP_01.pdf}
 \caption{The two point function for holographic CFT ($c \rightarrow \infty$) on UHP with two different channels which is decided by the cross ratio between $z_1,z_2$. }\label{UHP_plot}
\end{figure}
From the entropy on the UHP, we can find the corresponding bulk entropy we need after taking the conformal transformation to physical coordinate system by
\begin{equation}
 S_{\text{Bulk}} = S_{\Omega^{-2}g} = S_{\text{UHP}}- \frac{c}{6} \sum_{i} \log \Omega_i \,,
\end{equation}
where the sum runs over all the endpoints of intervals we considered.
Similar to the profile of dilaton, the bulk entropy is also sensitive to the location of the endpoints of the intervals. Before the shock, the possible contributions to generalized entropy is also divided into two different phases according to the position of endpoints. After the shock, the cross-ratio is fixed to be $1$ at the leading order. First, we study the similar problem in~\cite{Almheiri:2019psf} where they consider the generalized entropy for the interval with one point in the $\text{AdS}_2$ and another point on the boundary.
\subsection{Two points: AdS-bath}
We start from the simple case with only two points
\begin{equation}
 \begin{split}
  \text{AdS}_2, \text{before}\, \quad &x^{\pm}_2 :  x^+_2 >0, x^-_{2}<0 \,,  \text{or} \quad \text{after}\quad   x^+_2 >0, x^-_{2}>0\,,\\
  \text{bath},\text{after} \, \quad  &y_{1}^{\pm} : y^+_1>0, y^-_1>0 \,.
 \end{split}
\end{equation}
In order to parameterize the distance from the bath point to AdS boundary, we can choose the parametrization $y^{+}_1=u-y_0, y^-_1 = u+y_0$ where $y_0$ characterizes the distance to boundary.
From the above holographic formula for entanglement entropy with two points,
we can fix the choice of bulk entropy by taking account of the cross-ratio decided by the position of $\text{AdS}_2$ point, \ie
\begin{equation}
 S_{\Omega^{-2}g}=\left\{\begin{array}{ll}
  \frac{c}{6} \log \( \frac{|z_1-\bar{z}_1|\cdot|z_2 -\bar{z}_2|}{\Omega_1 \Omega_2} \)\,, & \zeta \in (\frac{1}{2}, 1)\,, {x^{-}_2<0<t<x^{+}_2} \\
  \,                                                                                                                                             \\
  \frac{c}{6} \log \( \frac{|z_1-z_2|\cdot|\bar{z}_1 -\bar{z}_2|}{\Omega_1 \Omega_2} \)\,, & \zeta \in (0,\frac{1}{2})\,, {x^{-}_2<0<t<x^{+}_2}  \\
  \,                                                                                                                                             \\
  \frac{c}{6} \log \( \frac{|z_1-z_2|\cdot|\bar{z}_1 -\bar{z}_2|}{\Omega_1 \Omega_2} \)\,, & \,, \zeta=0\,,{0<x_2^{-}<t<x_2^{+}} \,.
 \end{array}\right.
\end{equation}
First, for the point before the shock, it is obvious that we would have two different phases. The entropy in the first phase with $\zeta \ge  \frac{1}{2}$ is simply factorized to sum of contributions from the two endpoints  respectively, \ie
\begin{equation}
 S_{\Omega^{-2}g} (\zeta \ge  \frac{1}{2}) = \frac{c}{6} \(   \log \( \frac{|z_1-\bar{z}_1|}{\Omega_1 } \) + \log \( \frac{|z_2 -\bar{z}_2|}{ \Omega_2} \)  \) \,.
\end{equation}
For one point contribution, we would like to stress that the point before and after the shock have very different results
\begin{equation}
 S_{\Omega^{-2}g} ( y^{\pm}) =
 \begin{cases}
  \frac{c}{6} \log 2\,, \qquad    x^- <0\,,                                                                                 \\
  \frac{c}{6} \log  \left(\frac{24 E_{S}}{\epsilon c} \frac{y^- f(y^+)}{\sqrt{f^{\prime}(y^+)}}\right) \,, \qquad x^- >0\,, \\
 \end{cases}
\end{equation}
We need to find the QES by minimizing the generalized entropy with bulk entropy taking from one of the above term, \ie
\begin{equation}
 \partial_{x^{+}} S_{\text{gen}} =0 \,, \qquad \partial_{x^{-}} S_{\text{gen}} =0\,,
\end{equation}
and decide the position of endpoint in $\text{AdS}_2$ where we set it as $x^{\pm}$ or $y^{\pm}$.  As a summary, we need to take account of the dilaton from~\eqref{dilaton01} or~\eqref{dilaton02} and the following bulk entropy
\begin{equation}\label{bulk_entropy}
 S_{\text{Bulk}}=\left\{\begin{array}{ll}
  \frac{c}{6} \log \left(\frac{24 E_{S}}{\epsilon c} \frac{y_1^- f(y_1^+)}{\sqrt{f^{\prime}(y_1^+)}}\right)\,,(\text{A})                                                                        & \zeta \in (\frac{1}{2}, 1)\,, {x^{-}<0<t<x^{+}} \\
  \,                                                                                                                                                                                                                                              \\
  \frac{c}{6} \log \left(\frac{24 E_{S}}{\epsilon c} \frac{y_1^- x^-\(f(y_1^+)-x^+\)}{(x^+-x^-)\sqrt{f^{\prime}(y_1^+)}}\right)\,,(\text{B})                                                    & \zeta \in (0,\frac{1}{2})\,, {x^{-}<0<t<x^{+}}  \\
  \,                                                                                                                                                                                                                                              \\
  {\frac{c}{6} \log \left[\frac{2\left(y_1^--y^{-}\right)\left(x^{+}-f(y_1^+)\right)}{\epsilon\left(x^{+}-x^{-}\right)} \sqrt{\frac{f^{\prime}(y^-)}{f^{\prime}(y_1^+)}}\right]} \,, (\text{C}) & \zeta=0\,,{0<x^{-}<t<x^{+}}\,,
 \end{array}\right.
\end{equation}
where the cross ration is defined as
\begin{equation}
 \zeta = \frac{ x^- (f(y_{1}^+ )-x^+))}{x^+ (f(y_{1}^+ )- x^-)} \,,
\end{equation}
\textcolor{blue}{Even we find the holographic CFT has a sharp transition at $\zeta = \frac{1}{2}$, later we will see the transition between the two phases for generalized entropy may happen at other point because the QES is defined at the branch with the minimal entropy. }
Before we move to finding the solutions of QES, let's first comment on the effect by taking the one point from the $\text{AdS}_2$ boundary $(y_1^- \sim u \sim y_1^+)$ to the bath region, \ie
\begin{equation}
 u \longrightarrow  y^-_1=u+y_0\,, y^+_1=u-y_0 \,.
\end{equation}
it is obvious this operation has nontrivial effect on the QES surface and bulk entropy because the entropy in tall three cases all depend on both $y^{\pm}_1$. However, the effect from $u+y_0$ only appear at one term
\begin{equation}
 \log \( y_1^-\)  \quad \text{for}\quad  {x^{-}<0<t<x^{+}}\,, \qquad \log \( y_1^--y_-\)  \quad \text{for} \quad {0<x^{-}<t<x^{+}}\,.
\end{equation}
if the above contribution is negligible, it is easy to claim that the effect from moving the endpoint to the bath corresponds to reparameterize the QES by change $u$ to $u-y_0$.
\subsubsection{QES: Before the Shock}
\begin{figure}[t]
 \centering\includegraphics[width=3.00in]{QES_before.pdf}
 \caption{The evolution of QES. The arrow indicates the flow of the endpoint of QES with the time $t$, $u$. The Blue line is the physical solutions we considered in the paper. The green one is another branch of solution with larger entropy. Here we choose a large $k$ to make the deviation from horizon much more obvious.}\label{QES_plot}
\end{figure}
For the one endpoint in $\text{AdS}_2$ before the shock, we only need the static profile of dilaton~\eqref{dilaton01} and bulk entropy from the first two formulas in~\eqref{bulk_entropy}.
It easy to find the QES from bulk entropy with $\zeta \ge \frac{1}{2}$ is fixed to be the bifurcation point due to
\begin{equation}
 \partial_{x^+} S_{\text{gen}} = \frac{\partial_{+}  \phi}{4\GN }= \frac{\bar{\phi}_r}{4 \GN } \( \frac{2((\pi T_0 x^-)^2-1)}{ (x^+-x^-)^2} \)=0\,, \partial_{x^-} S_{\text{gen}} =\frac{\bar{\phi}_r}{4 \GN } \( \frac{2(1-(\pi T_0 x^+)^2)}{ (x^+-x^-)^2} \)=0
\end{equation}
only has one solution
\begin{equation}
 x^{\pm}= \pm \frac{1}{\pi T_0}
\end{equation}
which is nothing but the bifurcation point for original black hole with temperature $T_0$. The simplicity originates from the fact that the bulk entropy from holographic CFT with $\zeta \ge \frac{1}{2}$ does not depend on another endpoint in $\text{AdS}$, \ie $x^{\pm}$.  So we will have the generalized entropy at this phase
\begin{equation}
 S_{\text{gen,A}} \(\zeta \ge  \frac{1}{2}\)= \frac{\bar{\phi}_r}{4 \GN } \(  2\pi T_0    + 2k \log \left(\frac{24 E_{S}}{\epsilon c} \frac{y_1^- f(y_1^+)}{\sqrt{f^{\prime}(y_1^+)}}\right)\) \,.
\end{equation}
This solution is relevant only when
\begin{equation}
 \zeta_{\text{A}} = \frac{  1- \pi T_0 f(y_{1}^+)}{ \pi T_0f(y_{1}^+ )+1}\ge  \frac{1}{2}\,, \quad \longrightarrow \quad  f(y_1^+) \le \frac{1}{3\pi T_0}\,,
\end{equation}
which constrains the effective region parametrized by $y^+_1 = u-y_0 \le f^{-1}(\frac{1}{3\pi T_0})$.

Except for the first phase, we also have another phase with $\zeta \le  \frac{1}{2}$. The QES is derived from the non-trivial conditions
\begin{equation}
 \begin{split}
  \frac{4\GN }{\bar{\phi_r}}\partial_{+} S_{\text{gen}}  &=  \frac{2((\pi T_0 x^-)^2-1)}{ (x^+-x^-)^2}  +  2k \frac{x^- - f(y^+_1)}{ (f(y_1^+)-x^+)(x^+-x^-)}=0\,, \\
  \frac{4\GN }{\bar{\phi_r}}\partial_{-} S_{\text{gen}}  &=  \frac{2(1-(\pi T_0 x^+)^2)}{ (x^+-x^-)^2}  +   \frac{2k x^+}{ x^-(x^+-x^-)}=0\,,
 \end{split}
\end{equation}
which is reduced to the case with one pint at the boundary of $\text{AdS}_2$ if we set all $f(y^+_1) = f(u) =t$. Thanks to the simple profile of dilaton before the shock, the above equations are easily to be solved with \textcolor{blue}{\bf physical solutions} \footnote{The above equations actually have several branches of solutions. Here we only take the solutions satisfying the constrains and also have a smaller entropy. One can find another solution (the green curve shown in figure~\ref{QES_plot}) satisfying the constrains $x^-<0< x^+$, however its entropy is alway larger than that we show here. }
\begin{equation}\label{full_QES01}
 \begin{split}
  x^+ (f) &= \text{complicated form} \\
  x^-(f) &= \text{complicated form} \,,
 \end{split}
\end{equation}
which is simplified as
\begin{equation}\label{k_QES_02}
 \begin{split}
  x^+ (y_1^+) &= \frac{1}{\pi  T_0}-\frac{k}{\pi ^2 T_0^2}+\frac{k^2 \left(3 \pi  T_0 f\left(y^+_1\right)-1\right)}{2 \pi ^3 T_0^3 \left(\pi  T_0 f\left(y^+_1\right)-1\right)}+\mathcal{O}(k^3)\,,\\
  x^-(y_1^+) &= -\frac{1}{\pi  T_0}-\frac{k \left(\pi  T_0 f\left(y^+_1\right)+1\right)}{\pi ^2 T_0^2 \left(\pi  T_0 f\left(y^+_1\right)-1\right)}+\frac{k^2 \left(\pi  T_0 f\left(y^+_1\right)+1\right)}{2 \pi ^3 T_0^3 \left(\pi  T_0 f\left(y^+_1\right)-1\right)} + \mathcal{O}(k^3)\,,
 \end{split}
\end{equation}
where we use the small $k$ expansion and keep the first three orders. The small $k$ expansion is a good approximation for the early time region, which is broken when $ku \gg1$ due to the appearance of factor $e^{ku}$. With the exact solutions for $x^{\pm}$, we can easily find the generalized entropy in this phase which is shown in  figure~\ref{fig:Sgen01}. From the simple $k$ expansion, we can also derive the leading contributions to generalized entropy as
\begin{equation}\label{Sgen_before_k}
 \begin{split}
  S_{\text{gen,B}} \(\zeta \le  \frac{1}{2}\)&\approx \frac{\bar{\phi}_r}{4 \GN } \bigg[  2\pi T_0 + 2\pi T_1 (u-y_0)   + 2k \log \left(\frac{24 E_{S}}{\epsilon c}\frac{(u+y_0)}{2 \pi T_0 }  \right) \\
   & + 2k \log \left(\frac{\left(\pi  T_0 t_{\infty} \left(2 e^{-2 \pi  T_1 (u-y_0)}-1\right)+1\right)}{2\sqrt{\pi T_1 t_{\infty}} }\right)\bigg] + \mathcal{O}(k^2) \,,\\
 \end{split}
\end{equation}
where we only keep the first two leading order and the first line is the dominated term in this approximation because the second line is at order $\mathcal{O}\(k \log\(\frac{T_1-T_0}{T_1} \)\)$.  From this approximation, it is easy to find the almost linear behavior on time $u$ at the region $ 1 \ll u < \frac{1}{k}$ as shown in  figure~\ref{fig:Sgen01}.  For very late time $u > \frac{1}{k}$, you can expect the linear dependence on time $u$ is broken where the generalized entropy is described by another formula
\begin{equation}
 \begin{split}
  S_{\text{gen,B}} \(\zeta \le  \frac{1}{2}; ku> 1\)&\approx   \frac{\bar{\phi}_r}{4 \GN } \bigg[  2\pi T_0 + 2k \log \left(\frac{24 E_{S}}{\epsilon c}\frac{(u+y_0)}{\sqrt{f^{\prime}(u-y_0)}}  \right)  +C\bigg]  \,,
 \end{split}
\end{equation}
where the constant $C$ is fixed by taking the $u$ to infinity and the bulk term is dominated by the log term rather the previous linear term.
Similarly, this phase is only relevant only when the condition on cross ratio is satisfied
\begin{equation}
 \zeta_{\text{B}} =\frac{ x^- (y_{1}^+ )(f(y_{1}^+ )-x^+(y_{1}^+ )))}{x^+(y_{1}^+ ) (f(y_{1}^+ )- x^-(y_{1}^+ ))}\,.
\end{equation}
After fixing the saddle point from the two entanglement entropy before the shock~\eqref{bulk_entropy}, we also need to decide the which one really represents the QES. First of all, all the two solutions is constrained by the cross ratios.  And we can also find the A, B phase will intersect at time $u_{AB}$ (or $y_{1,AB}^-$ for bath point).  So there are three transition points we need to consider
\begin{equation}
 \begin{split}
  \zeta_{\text{B}} &=\frac{1}{2} \qquad \text{at} \qquad  u_{B} \,,\\
  S_{\text{gen,B}} &=S_{\text{gen,A}}\qquad \text{at} \qquad  u_{AB} \,,\\
  \zeta_{\text{A}} &=\frac{1}{2} \qquad \text{at} \qquad  u_{A}\,, \\
  \text{with}\qquad & u_B < u_{AB} <u_{A} \,.
 \end{split}
\end{equation}
where the three transition point are more and more near when $k$ is smaller and smaller. (\smr{Add analytical descriptions to that point}) From this, it is easy to see that the real QES is the A branch before the transition time $u_{AB}$ and then jumps \footnote{The endpoint point of QES jumps from bifurcation point $x^{\pm}=\pm\frac{1}{\pi T_0}$ to another point $x^{\pm} (y^+_{1,AB})$ before the shock.} to the B branch with smooth transition on generalized entropy from $S_{\text{gen,A}}$ to $S_{\text{gen,B}}$.



\begin{figure}[t]
 \includegraphics[width=0.48\textwidth]{Sgen_before00.pdf} \hspace{0.01\textwidth}
 \includegraphics[width=0.48\textwidth]{Sgen_before_002.pdf}
 \caption{The generalized entropy evaluated using the full solutions. The blue curve is derived from~\eqref{full_QES01}. The green one represents the generalized entropy with endpoint at bifurcation point. We also draw the plot for generalized entropy from non-holographic formula. The green point in the right plot indicates the point $\zeta=\frac{1}{2}$ for the $\zeta \le \frac{1}{2}$ phase. \smr{Need to be updated. Add $u_{AB}$, $u_A$.}}
 \label{fig:Sgen01}
\end{figure}

\subsubsection{QES: after the Shock}
\begin{figure}[t]
 \includegraphics[width=0.54\textwidth]{QES_after_xp.pdf} \hspace{0.01\textwidth}
 \includegraphics[width=0.48\textwidth]{QES_after_ym.pdf}
 \caption{The numerical solutions $x^{+}, y^-$ from eqs.~\eqref{QES_equations} is presented by the dotted lines. Note that the left plot is a log plot. The solid line are the linear approximation from~\eqref{}. }
 \label{fig:QESxpym}
\end{figure}
When the endpoint move to the region in $\text{AdS}_2$ after the shock, the bulk entropy is defined in~\eqref{bulk_entropy} with C. This case is same as that analyzed in~\cite{Almheiri:2019psf}. The QES is derived from the solutions of the following  two equations
\begin{equation}\label{QES_equations}
 \begin{split}
  \frac{4\GN }{\bar{\phi_r}}\partial_{+} S_{\text{gen}}  &=  \frac{2(\pi T_0 x^-)^2-2-k \int_{0}^{x^-} (x^- -t)^2\{u,t\}\, dt  }{ (x^+-x^-)^2}  +  2k \(\frac{1}{ x^+-f(y_1^+)} - \frac{1}{x^+-x^-} \) =0\,, \\
  \frac{4\GN }{\bar{\phi_r}}\partial_{-} S_{\text{gen}}  &=  \frac{2-2(\pi T_0 x^+)^2+k \int_{0}^{x^-} (x^+ -t)^2\{u,t\}\, dt   }{ (x^+-x^-)^2}  \\
  &\qquad +2k \( \frac{1}{x^+-x^-}  -\frac{1}{(y_1^--y^-)f^{\prime}(y^-)} + \frac{f^{\prime\prime}(y^-)}{2(f^{\prime}(y^-))^2} \)=0\,.
 \end{split}
\end{equation}
Because of the integral in the dilaton term, it is not easy fo find the analytical solutions for these equations. So first, we show the results from numerics and presents the approximate solutions in interesting regions. The full answer is presented in the following figure~\ref{fig:QESxpym} and the corresponding generalized entropy is shown in figure~\ref{fig:pagecurve}.

\begin{figure}[t]
 \centering\includegraphics[width=3.80in]{page_curve.pdf}
 \caption{The dotted pink line shows the numerical results for generalized entropy with endpoint after the shock. The page time is indicated by the green point in this plot.}\label{fig:pagecurve}
\end{figure}

From the numerical plot, it is interesting to find that around the page time the two branch both presents linear behavior. For generalized entropy before the page time, its linearity is illustrated by approximation from the small $k$ expansion in~\eqref{Sgen_before_k}. For the generalized entropy, we would also like to use simple analytical results to show this linear property. The approximation is exactly done in the original paper~\cite{Almheiri:2019psf} by carefully dealing with the integral with Schwarzian. The key point is we can use the approximation for coordinate map function around small $k$ with fixed $ku$
\begin{equation}
 \log \left(\frac{t_{\infty}-f(u)}{2 t_{\infty}}\right) \sim-\frac{4 \pi T_{1}}{k}\left(1-e^{-\frac{k}{2} u}\right)+O\left(k e^{\frac{k}{2} u}\right) \,,
\end{equation}
the limits in the region around page time ( $u \le \frac{1}{k}$)
\begin{equation}
 e^{-ku} \approx 1- ku + \frac{1}{2}(ku)^2 + \mathcal{O}(k^3)\,,
\end{equation}
and notice the fact $x^+ \sim t \sim x^-$ but they satisfy  the following conditions  \footnote{We can easily see that from our numerical results.}
\begin{equation}
 x^+ \approx  t_{\infty}\,, \quad x^+ -t \ll t-x^- \approx x^+-x^-  \approx t_{\infty}  -x^- \,.
\end{equation}
Finally, we can keep the leading term in the QES equations and arrive at these extremely simple equations
\begin{equation}
 \begin{split}
  0&=\frac{4\GN }{\bar{\phi_r}}\partial_{+} S_{\text{gen}}  \approx 4\pi T_1 \frac{e^{-\frac{k}{2} y^-}}{t_{\infty}-x^-} - \frac{2k}{ x^+ -t} \,, \\
  0&=\frac{4\GN }{\bar{\phi_r}}\partial_{-} S_{\text{gen}}  \approx  \frac{1}{(x^+-x^-)^2} \( 4\pi T_1 (t_{\infty}-x^+) e^{-\frac{k}{2}y^-}   + \frac{k}{2} (t_{\infty}-x^-) \) \,,
 \end{split}
\end{equation}
whose solution is easily to be derived as

\begin{equation}
 \begin{split}
  x^+  &= \frac{4}{3} t_{\infty} -\frac{1}{3} t + \mathcal{O}(k)\,,\\
  y^- &= u -\frac{t_{\infty}}{2} \log \( \frac{8\pi T_1}{3k} \)+ \mathcal{O}(k)\,.
 \end{split}
\end{equation}
Th above linear solution have captured the leading order behavior of QES and also the generalized entropy. We compare the linear solutions to that from numerics at figure~\ref{fig:QESxpym}. The linear generalized entropy around page time $u_{\text{page}}$ is described by
\begin{equation}
\begin{split}
S_{\text{gen,C}} & \approx   \frac{\bar{\phi}_r}{4 \GN } \[  2\pi T_1 - k \pi T_1 (u-C) + 2k \( \log \( \frac{8}{3\epsilon} \) -C +\log C + kC  \) +\mathcal{O}(k^2) \]\,,
\end{split}
\end{equation}

\subsubsection{Comparison with Free CFT theory}
Similar results except for the very early time.
\begin{figure}[t]
 \centering\includegraphics[width=3.80in]{Sgen_free01.pdf}
 \caption{The page with bulk entropy from free theory rather than holographic CFT.}\label{fig:Sgenfree}
\end{figure}





\subsection{Three points: AdS-bath-bath}

